Towards Verification of Constituent Systems through Automated Proof

This paper explores verification of constituent systems within the context of the Symphony tool platform for Systems of Systems (SoS). Our SoS modelling language, CML, supports various contractual specification elements, such as state invariants and operation preconditions, which can be used to specify contractual obligations on the constituent systems of a SoS. To support verification of these obligations we have developed a proof obligation generator and theorem prover plugin for Symphony. The latter uses the Isabelle/HOL theorem prover to automatically discharge the proof obligations arising from a CML model. Our hope is that the resulting proofs can then be used to formally verify the conformance of each constituent system, which is turn would result in a dependable SoS.

==> sections/discussion.tex <==
\section{Future work}
\label{sec:discussion}

In this paper, we have demonstrated the verification of constituent
system \emph{models}. An interesting issue would be the verification
of an actual implementation, with respect to realistic system
properties. Whilst clearly not in the scope of this paper, we would
consider the work of this paper in context with other system
engineering activities. In particular; positioning constituent system
verification with respect to the work of Holt et al~\cite{Holt12} on SoS
requirements engineering and
the specification of SysML contracts and translation to CML~\cite{Bryans2014a}
may provide the means to more realistic property verification.

The current CML theorem prover focuses on VDM-style proof obligations
which deal with issues such as subtyping and internal consistency. In
the future we will extend this with a more comprehensive calculus,
such as a Hoare logic~\cite{COMPASSD23.4d} or a weakest precondition
calculus, which would both expand on the existing proof
obligations. This would also allow us to reason directly about CML
process and state behaviour, and therefore provide fuller support for
reasoning about contracts.

Another extension to the proof obligations relates to  to scaling our approach
from the level of constituent systems to the \ac{sos} level, thus ensuring that
the verified constituent systems  interact in a manner that ensures the desired
behaviour of the overall \ac{sos}.

Just as pre-conditions and invariants can be used to specify the
properties that the \ac{pog} and \ac{tpp} verify, we need a mechanism
that allows these tools to reason about correctness at the \ac{sos}
level. We see two distinct possibilities here: the first is to
introduce a new \ac{cml} construct that allows one to specify
invariants over the entire \ac{sos}, thus being able to ``see'' inside
all constituents. The second approach is to take the existing \acp{po}
that verifies a system and use them to also verify the interface of a
constituent. Afterwards, one must establish a means by which these
verified interfaces can be combined to establish global \ac{sos}
properties.  Of the two approaches, the second one seems closer to the
spirit of \ac{sos} engineering, and we believe CS refinement provides
a way forward here.

We are also currently working on a tool for CS refinement, which
combines with the theorem prover and can be used to formally
demonstrate contractual satisfaction. This will reuse the \ac{pog} to
enumerate and discharge refinement provisos which must often be
satisfied to ensure validity of a refinement step. Refinement will be
principally supported by Isabelle, though we are also exploring the
use of model generation tools to aid automation. For example, the
Maude rewriting logic engine~\cite{Clavel2002187} has previously been
applied to automated refinement~\cite{griesmayer13refine}, which we
hope to adapt for CML. Such advances over the current technology are
feasible because of our extensible approach to semantics provided by
UTP.

Both plug-ins presented here are still at an early development stage. While the
\ac{tpp} and its associated Isabelle theories support a significant subset of
\ac{cml} (types, expressions, functions, and operations), work is ongoing on
increasing the coverage of the plug-in. The proof tactics are also under
further development in order to discharge increasingly complex goals. Moreover
we wish to expose more of Isabelle's native proof facilities in the \ac{tpp},
such as \textsf{sledgehammer} and \textsf{nitpick}, so as to bring their full
weight to bear in discharging or refuting proof obligations. Parallel to this
there is work to formalise the proof obligations in Isabelle with respect to
the \ac{cml} semantics. Finally, we hope to produce guidance to the user of how
to interpret failure when a PO cannot be discharged.


% Questions originally posed by reviews:
% \begin{itemize}
%    \item What parts of CML are particularly difficult to handle? 
%    \item Why are the proof obligations that refer to the current value of
%        state variables the ones that cannot easily be discharged
%        automatically? 
%    \item Is it because more powerful proof methods, like generalised
%        induction, are required to handle these?
%    \item What kind of proof methods are supported by the mentioned Isabelle
%        tactics? 
%    \item Does it pay off to use Isabelle for the theorem proving tasks, or
%        would other options provide more automation support?  
%     \item What types of proof obligations would be necessary to verify correct
%         interaction of constituent systems to ensure the desired behaviour of
%         the overall SoS? Will these be similar, or completely different?
%     \item  show in how far the model properties relate to the realistic system
%         and its properties - this includes a discussion of the type of system
%         requirements that can be treated and those that are outside the scope
%         of the approach (first order logic is not able to specify complex
%         dependability requirements - at least with regard to timing and
%         reactive properties)
% \end{itemize}

% Final list of questions for the paper (LDC):
% \begin{itemize}
%     \item What parts of CML are particularly difficult to handle, both from 
%         PO generation and automatic discharge POV?
%     \item What kinds of obligations can be used to verify the behavior
%         of the overall SoS? Particularly, is it possible to reason about emergent,
%         SoS properties without ``seing'' inside the constituents? Perhaps by
%         reasoning about SOS properties using properties of the CS. 
%     \item What can be said about the relation between model properties
%         and realistic system properties? Perhaps more of a general CML issue.
% \end{itemize}

% RJP suggested answers:

% As  mentioned in Section~\ref{sec:example}, the \ac{pog} and \ac{tpp} cover substantial parts of CML, however, the reactive elements: \emph{actions} and complex \emph{processes} have limited support. Of the areas covered, the \ac{tpp} finds \fbox{areas of difficulty}.

% \fbox{use para 3 in conclusion to answer the 2nd question. Also consider mentioning refinement of abstract sos model.}



==> sections/furtherwork.tex <==
\section{Further Work}
\label{sec:furtherwork}


The work presented here enables the verification of internal consistency and
other specified properties of a constituent system modelled in \ac{cml}.
However, these properties are expressed and considered at the level of a single
constituent system.

The next step is to ensure that these verifiend constituent systems are interacted
with in a manner that ensures their correct behavior. Just as pre-conditions are used
to ensure functions are called with the correct arguments, one needs a mechanism
to ensure that any inputs offered to a constituent system are valid.

In essence, we plan to use \ac{po} to offer a formally verified interface for 
a constituent such that any other constituent in the \ac{sos} can rely on the
verified constituent to behave as specified.

Parallel to this, there is also ongoing work to verify the correctness of the
\acp{po} with respect to the formal \ac{cml} semantics, facilitated by our deep
embedding.




